Deflated HeteroPCA: Overcoming the curse of ill-conditioning in heteroskedastic PCA

This paper is concerned with estimating the column subspace of a low-rank matrix $\boldsymbol{X}^\star \in \mathbb{R}^{n_1\times n_2}$ from contaminated data. How to obtain optimal statistical accuracy while accommodating the widest range of signal-to-noise ratios (SNRs) becomes particularly challenging in the presence of heteroskedastic noise and unbalanced dimensionality (i.e., $n_2\gg n_1$). While the state-of-the-art algorithm $\textsf{HeteroPCA}$ emerges as a powerful solution for solving this problem, it suffers from "the curse of ill-conditioning," namely, its performance degrades as the condition number of $\boldsymbol{X}^\star$ grows. In order to overcome this critical issue without compromising the range of allowable SNRs, we propose a novel algorithm, called $\textsf{Deflated-HeteroPCA}$, that achieves near-optimal and condition-number-free theoretical guarantees in terms of both $\ell_2$ and $\ell_{2,\infty}$ statistical accuracy. The proposed algorithm divides the spectrum of $\boldsymbol{X}^\star$ into well-conditioned and mutually well-separated subblocks, and applies $\textsf{HeteroPCA}$ to conquer each subblock successively. Further, an application of our algorithm and theory to two canonical examples -- the factor model and tensor PCA -- leads to remarkable improvement for each application.

==> analysis.tex <==
\section{Analysis}\label{sec:proof_sketch}
In this section, we briefly explain the proof strategy of Theorem \ref{thm:two_to_infty}. The proof of Theorem \ref{thm:spectral} is similar to proving the spectral norm error bound in Theorem \ref{thm:two_to_infty}. Recall that $\bm{U}_k$ is the rank-$r$ leading singular space of $\bm{G}_k$, the matrix whose off-diagonal entries are equal to those for $\bm{Y}\bm{Y}^\top$ and whose diagonal entries are imputed by applying the {\sf HeteroPCA} after the $k$-th round. By sequentially performing the {\sf HeteroPCA}, we expect the diagonal entries of $\bm{G}_k$ to get closer to those of $\bm{Y}\bm{Y}^{\top} - \mathcal{P}_{\sf diag}(\bm{E}\bm{E}^{\top})$, an unbiased estimator for $\bm{X}^\star\bm{X}^{\star\top}$. Inspired by this intuition, we let 
\begin{align}\label{eq:U_oracle}
	\bm{U}^{\sf oracle} =  \text{ the leading } r \text{ eigenvectors of } \bm{M}^{\sf oracle},
\end{align}
where
\begin{align}\label{eq:M_oracle}
	\bm{M}^{\sf oracle}
	&:=\bm{Y}\bm{Y}^{\top} - \mathcal{P}_{\sf diag}\left(\bm{E}\bm{E}^{\top}\right) + \mathcal{P}_{\sf diag}\left(\bm{E}\bm{V}^\star\bm{V}^{\star\top}\bm{E}^\top\right)\notag\\
	&=\left(\bm{U}^{\star}\bm{\Sigma}^{\star} + \bm{E}\bm{V}^{\star}\right)\left(\bm{U}^{\star}\bm{\Sigma}^{\star} + \bm{E}\bm{V}^{\star}\right)^\top + \mathcal{P}_{\sf off\text{-}diag}\left(\bm{E}\bm{E}^\top - \bm{E}\bm{V}^\star\bm{V}^{\star\top}\bm{E}^\top\right)\notag\\
	&=\widetilde{\bm{U}}\widetilde{\bm{\Sigma}}^2\widetilde{\bm{U}}^\top + \bm{Z}.
\end{align}
Here, $\widetilde{\bm{\Sigma}} = {\sf diag}(\widetilde{\sigma}_1, \dots, \widetilde{\sigma}_r) \in \bbR^{r \times r}$ is the diagonal matrix containing all singular values of $\bm{U}^{\star}\bm{\Sigma}^{\star} + \bm{E}\bm{V}^{\star}$ (in decreasing order) and $\widetilde{\bm{U}} \in \mathcal{O}^{n_1, r}$ is its corresponding column subspace, $\bm{Z} = \mathcal{P}_{\sf off\text{-}diag}(\bm{E}\bm{E}^\top - \bm{E}\bm{V}^\star\bm{V}^{\star\top}\bm{E}^\top)$. Rather than proving that $\bm{U}$ and $\bm{U}^\star$ are close directly, we will upper bound the distances between $\bm{U}^{\sf oracle}$ and $\bm{U}^\star$, then $\bm{U}$ and $\bm{U}^{\sf oracle}$, separately. Specifically, we will show that
\begin{itemize}
	\item[1.] with high probability, 
	\begin{subequations}
		\begin{align}
			\left\|\bm{U}^{\sf oracle}\bm{U}^{\sf oracle\top} - \bm{U}^\star\bm{U}^{\star\top}\right\| &\lesssim \frac{\sqrt{n_1n_2}\omega_{\sf max}^2\log^2 n}{\sigma_r^{\star2}} + \frac{\sqrt{n_1}\omega_{\sf max}\log n}{\sigma_{r}^\star},\label{ineq:oracle_spectral}\\
			\left\|\bm{U}^{\sf oracle}\bm{U}^{\sf oracle\top} - \bm{U}^\star\bm{U}^{\star\top}\right\|_{2,\infty} &\lesssim \sqrt{\frac{\mu r}{n_1}}\left(\frac{\sqrt{n_1n_2}\omega_{\sf max}^2\log^2 n}{\sigma_r^{\star2}} + \frac{\sqrt{n_1}\omega_{\sf max}\log n}{\sigma_{r}^\star}\right)\label{ineq:oracle_two_to_infty}.
		\end{align}
	\end{subequations}
	\item[2.] with high probability, for all $1 \leq k \leq k_{\sf max}$,
	\begin{align}\label{ineq58}
		\left\|\bm{U}_k\bm{U}_k^{\top} - \bm{U}_k^{\sf oracle}\bm{U}_k^{\sf oracle\top}\right\| \lesssim \sqrt{\frac{\mu r}{n_1}}\frac{\left(\sqrt{n_1n_2} + n_1\right)\omega_{\sf max}^2\log^2 n + \sigma_{r_k + 1}^{\star2}}{\sigma_{r_k}^{\star2} - \sigma_{r_{k+1}}^{\star2}},
	\end{align}
	where $\bm{U}_k^{\sf oracle} = (\bm{U}^{\sf oracle})_{:, 1: r_k}$ and $\bm{U}_k = \bm{U}_{:, 1: r_k}$.
\end{itemize}
The second part, \eqref{ineq58}, is true if we can bound the difference between diagonal entries of $\bm{M}^{\sf oracle}$ and $\bm{G}_k$, which can be shown by induction. Turning back to the first part, we let $\widetilde{\bm{U}}\widetilde{\bm{\Sigma}}^2\widetilde{\bm{U}}^\top$ be the SVD of
$$\left(\bm{U}^{\star}\bm{\Sigma}^{\star} + \bm{E}\bm{V}^{\star}\right)\left(\bm{U}^{\star}\bm{\Sigma}^{\star} + \bm{E}\bm{V}^{\star}\right)^\top$$ and let $\bm{Z}$ denote the ``noise matrix'' $\mathcal{P}_{\sf off\text{-}diag}(\bm{E}\bm{E}^\top - \bm{E}\bm{V}^\star\bm{V}^{\star\top}\bm{E}^\top).$ Some calculation shows that $\widetilde{\bm{U}}\widetilde{\bm{U}}^{\sf oracle\top} - \bm{U}^\star\bm{U}^{\star\top}$ is small in terms of $\ell_2$ and $\ell_{2,\infty}$ errors and thus we only need to bound $\|\bm{U}^{\sf oracle}\bm{U}^{\sf oracle\top} - \widetilde{\bm{U}}\widetilde{\bm{U}}^{\top}\|$ and $\|\bm{U}^{\sf oracle}\bm{U}^{\sf oracle\top} - \widetilde{\bm{U}}\widetilde{\bm{U}}^{\top}\|_{2,\infty}$. The spectral norm error bound can be established by Davis-Kahan Theorem. 




The $\ell_{2,\infty}$ error bound, however, is much more difficult to prove. To achieve a sharp and condition-number-free bound,  we apply the following spectral representation lemma \citep{xia2021normal}, which was proposed for subspace inference under i.i.d.~noise and allows us to bound an infinite sum of (exponentially decayed) two-to-infinity norms instead of dealing with $\|\bm{U}^{\sf oracle}\bm{U}^{\sf oracle\top} - \widetilde{\bm{U}}\widetilde{\bm{U}}^{\top}\|_{2,\infty}$ directly.






Set $\overline{\bm{U}} = \bm{\widetilde{U}}$ and $\overline{\bm{M}} = \widetilde{\bm{U}}\widetilde{\bm{\Sigma}}^2\widetilde{\bm{U}}^\top$. For $k > \log n$, one can show that the terms in \eqref{ineq:representation} decay exponentially and thus can be easily bounded. When it comes to $1 \leq k \leq \log n$, we derive sharp bounds on $\|[\mathcal{P}_{\sf off\text{-}diag}(\bm{E}\bm{E}^\top)]^k\bm{E}\bm{V}^\star\|_{2,\infty}$ and $\|[\mathcal{P}_{\sf off\text{-}diag}(\bm{E}\bm{E}^\top)]^k\bm{U}^\star\|_{2,\infty}$ (see Lemmas \ref{lm:error_moment1} and \ref{lm:error_moment2} for details) and upper bound the $k$-th term in \eqref{ineq:representation} by induction. Combining these facts, we arrive at \eqref{ineq:oracle_spectral} and \eqref{ineq:oracle_two_to_infty} . 
A formal statement is shown in Theorem \ref{thm:oracle}. This together with \eqref{ineq58} and the (near) equivalence of subspace distances finishes the proof of Theorem \ref{thm:two_to_infty}.







